Model Checkers Are Cool: How to Model Check Voting Protocols in Uppaal

The design and implementation of an e-voting system is a challenging task. Formal analysis can be of great help here. In particular, it can lead to a better understanding of how the voting system works, and what requirements on the system are relevant. In this paper, we propose that the state-of-art model checker Uppaal provides a good environment for modelling and preliminary verification of voting protocols. To illustrate this, we present an Uppaal model of Pr\^et \`a Voter, together with some natural extensions. We also show how to verify a variant of receipt-freeness, despite the severe limitations of the property specification language in the model checker.

==> model_old.tex <==
%\documentclass[
%]{article}

%\usepackage{enumitem}
%\usepackage{indentfirst}
%\usepackage{amssymb,amsmath}


%\begin{document}


\section{Model overview}\label{model-overview}

In this section we will give a detailed description on each model
component, its elements and their common interactions. In case of more
than one instance of a component type, an identifier (starting from 0)
will be associated with each instance. 

\subsection{Global (shared) scope}\label{global-shared-scope}  

For better code manageability we define some simple data structures
available to every model component:
\begin{itemize}[nosep]
\item \textbf{PK} - ElGamal public key, constisting of
three integers: cyclic group order \texttt{p}, generator \texttt{a} and
\texttt{b\ =\ a\^{}k}, where \texttt{k} is a private key. 

\item \textbf{Ciphertext} - a pair of integers \texttt{y1} and \texttt{y2},
which represent an instance of ElGamal cipher. A plaintext \texttt{m}
encrypted with public key \texttt{T} with randomness \texttt{y} will be
noted as \texttt{E\_T(m,y)}, if the value of \texttt{y} is not
set/known, then it will be noted as \texttt{E\_T(m,*)} instead.

\item \textbf{Ballot} - a pair of onion \texttt{o\ =\ E\_T(s,*)} and candidate
list \texttt{cl\ =\ pi(s)}, , where \texttt{s} is a seed associated with
the ballot and \texttt{pi} is a function which associates a seed to some
permutation of the candidates \texttt{pi:\ R\ -\textgreater{}\ Perm(C)}.

\item \textbf{Receipt} - a pair of onion and an index of cell with X marked
by the Voter, to whom this receipt belongs. It can be used to verify if
Voter's choice was recorded and if it was done correctly.
\end{itemize}\medskip


\noindent Global read-only configuration variables:

\begin{itemize}[nosep]
\item \texttt{c\_total} - number of candidates

\item \texttt{v\_total} - number of voters 

\item \texttt{mt\_total} - number of mix tellers 

\item \texttt{dt\_total} - number of decryption tellers

\item \texttt{dt\_required} - number of dtellers needed 
to cooperate in order to decrypt the cipher

\end{itemize}\smallskip

\noindent From model configuration values we derive and precalculate some helper
variables, such as lists of possible reciept batch permuatations
\texttt{P\_b}, list of candidates permutations \texttt{P\_c}, list of
cyclic shifts of candidates \texttt{S\_c}, lookup table (based on seed
space) for onion and seed, which maps onion to its seed (+- all possible
candidate choices).\medskip

\noindent Global variables:
\begin{itemize}[nosep]
\item \texttt{curr\_phase} - encoded value of current phase of voting (0 =
ballot generation, 1 = voting, 2 = mixing, 3 = decryption, 4 = posting
results) 
\item \texttt{board} - 2 dimentional list of ciphertexts (world bulletin board), 
where first column is reserved for the batch of initial onions
(with absorbed index), next $(mt\_total\cdot2)$ columns store results
of mtellers, and remaining $dt\_required$ columns store results of dtellers
(only last one will store fully decrypted message) 
\item \texttt{mixes} - encodes the turn of next mteller (if any)
\item \texttt{decryptions} - number of decryptions made
\end{itemize}\medskip

There is also a set of globally shared variables used exclusively to simulate
the passing of value through the channel; use of those will be specified in 
transition description.

\subsection{Voter}\label{voter}

\noindent Private variables:
\begin{itemize}[nosep]
\item
  \texttt{receipt} - with each voter we associate a ballot, and later a receipt,
  which one gets after casting her vote
\item
  \texttt{coercion} - boolean value, indicating if coercer has established a
  contact with Voter
\item
  \texttt{chosen} - a number representation of prefered candidate
\end{itemize}\medskip

\noindent States: 
\begin{itemize}[nosep]
\item
  \emph{idle} - waiting for election phase
\item
  \emph{met\_coercer} - contacted by coercer
\item
  \emph{has\_ballot} - obtained the ballot form
\item
  \emph{marked\_choice} - marked an index of chosen candidate (and destroyed
  left hand side with candidate list)
\item
  \emph{received\_receipt} - after sending a copy, receipt is now 
  kept by the voter
\item
  \emph{shown\_receipt} - decided to show proof of vote (receipt) (?)
\item
  \emph{verification} - decided to verify the receipt
\item
  \emph{passed} - has a confirmation (without revealing any other information), that receipt appears
  correctly
\item
  \emph{failed} - has an evidence, that receipt either does not
  appear (?) or appears incorrectly (in case of index absorbtion both
  cases are the same)
\item
  \emph{end} - finish of voting ceremony
\item
  \emph{punished} - was punished by Coercer
\item
  \emph{not\_punished} - was not punished by Coercer
\end{itemize}\medskip

\noindent Transitions: 
\begin{itemize}[nosep]
\item
  \emph{idle$\rightarrow$met\_coercer}: enable synchronized transition,
  if taken, then set \texttt{coercion} to true
\item
  \emph{idle$\rightarrow$has\_ballot}
  (\emph{met\_coercer$\rightarrow$has\_ballot)}: if election phase
  started \texttt{curr\_phase==1}, then ballot can be obtained
\item
  \emph{has\_ballot$\rightarrow$marked\_choice}: find (procedure
  \texttt{c\_index}) and mark a cell \texttt{receipt.i} with with name
  of chosen candidate \texttt{X}
\item
  \emph{marked\_choice$\rightarrow$received\_receipt}: initialize
  synchronization and send the \texttt{receipt} to the server using
  \texttt{recorded} global variable.
\item
  \emph{received\_receipt$\rightarrow$shown\_receipt}: if was coercered
  ( \texttt{coercion==true} ), initialize the synchronized transition
  with Coercer over channel \texttt{show} and pass the value of
  \texttt{receipt} using \texttt{shown} global variable.
\item
  \emph{received\_receipt$\rightarrow$verification}
  (\emph{shown\_receipt$\rightarrow$verification}): if unprocessed
  results are published ( \texttt{curr\_phase\textgreater{}1} ), enable
  transition
\item
  \emph{received\_receipt ( shown\_receipt, passed, failed
  )$\rightarrow$end}: go to the end of voting ceremony
\item
  \emph{end$\rightarrow$punished}: if was coerced (
  \texttt{coercion==true} ) enable synchronized transition with Coercer
  over channel \emph{punish}
\item
  \emph{end$\rightarrow$not\_punished}: if was coerced (
  \texttt{coercion==true} ) enable synchronized transition with Coercer
  over channel \emph{not\_punish}
\end{itemize}


\subsection{Coercer}\label{coercer}

\noindent Private variables: 
\begin{itemize}[nosep]
\item
  \emph{coercion} - a boolean list to keep track coerced voters (more
  precisely if further interaction with one is possible,
  i.e.\textasciitilde can be punished or not) 
  \item \emph{seen} - a boolean
  list, which indicates whether coerced seent the proof of vote
\end{itemize}\medskip

\noindent There is only a single state called \emph{loop} for Coercer, which has 4 looping
transitions, altering private variables. A more common approach would
be cloning the state for every possible Boolean evaluation and then
recognizing the reachable subset of states. However, that would lead to loss
of generality and readability of the component (e.g.: for 3 voters
Coercer would have had $2^{3\cdot2}\ =\ 64$ states).\medskip

\noindent Transitions with respect to Voter \texttt{v\_id} (clockwise starting with top left): 
\begin{itemize}[nosep]
	\item Initialize synchronized transition with \texttt{v\_id} if
	  possible (if corresponding transition is enabled for \texttt{v\_id}) over channel \texttt{interact}
	  and update \texttt{coercion} list of coerced voters
	\item If \texttt{v\_id} was coerced, then enable synchronozed transition; 
	if it is taken, then update \texttt{seen[v\_id]} to true
	\item If \texttt{v\_id} was coerced, then initialize transition with \texttt{v\_id} over channel 
	\texttt{punish} and set \texttt{coercion[v\_id]} to false,
	  finalizing interaction between two
	\item If \texttt{v\_id} was coerced, then initialize transition with \texttt{v\_id} over channel \texttt{not\_punish} and set \texttt{coercion[v\_id]} to false, finalizing interaction between two.
\end{itemize}


\subsection{Mteller}\label{mteller}

\noindent Private variables:

\begin{itemize}[nosep]
	\item \texttt{rand\_factor} - 2 dimmensional integer list (size $2\times|V|$), 
	used to memorize which randomization factors were used during re-encryption 
	for further possible audit
	
	\item \texttt{link\_map }- 2 dimmensional integer list (size $2\times|V|$), 
	used to memorize which permutation was used during mixing for further possible
	audit
	 
	\item \texttt{rand\_vec }- (helper variable) integer list with random values
	
	\item \texttt{rand\_ptr }- (helper variable) index for \texttt{rand\_vec} elements
\end{itemize}\medskip


\noindent States:
\begin{itemize}[nosep]
\item \emph{idle} - waiting start of mixing phase 
\item \emph{odd} - performing the first mixing 
\item \emph{even} - performing the second mixing
\item \emph{audit} - wait and respond to auditor's requests 
\item \emph{halt} -passed the audit 
\item \emph{caught} - failed the audit, considered cheater
\end{itemize}\medskip


\noindent Transitions:

\begin{itemize}[nosep]

\item \emph{idle$\rightarrow$odd}: if mixing phase started
\texttt{curr\_phase==2} and it is current mteller's turn
(\texttt{mixes==mt\_id}), then enable transition; if it is taken, 
set \texttt{rand\_ptr} to zero 

\item \emph{odd$\rightarrow$odd}/\emph{even$\rightarrow$even}
(upper loop): if \texttt{rand\_ptr\ \textless{}\ v\_total}, then enable
transition and write randomness factor \texttt{r1} (chosen
non-deterministically) as an element \texttt{rand\_vec[rand\_ptr]}, 
increment \texttt{rand\_ptr} afterwards 

\item \emph{odd$\rightarrow$odd}/\emph{even$\rightarrow$even} (lower loop):
if \texttt{rand\_ptr\ ==\ v\_total}, then select permutation index
\texttt{r2} and perform re-encryption mix (\texttt{do\_mixing}), which will
increment \texttt{rand\_ptr} by 1. 

\item \emph{odd$\rightarrow$even}: if previous mix is
done (\texttt{rand\_ptr\textgreater{}v\_total}), enable transition; if
transition is taken, reset \texttt{rand\_ptr} for new randomness generation

\item \emph{even$\rightarrow$audit}: if previous mix is
done (\texttt{rand\_ptr\textgreater{}v\_total}), enable transition; if
transition is taken, pass the turn to tje next mteller incrementing 
\texttt{mixes} by 1 

\item \emph{audit$\rightarrow$audit} (left): enabled
synchronized transition with Auditor over channel \texttt{reveal\_left};
if taken, send randomization factor source index ($\pi^{-1}(term\_id)$)
for \texttt{term\_id} record

\item \emph{audit$\rightarrow$audit} (right):
enabled synchronized transition with Auditor over channel
\texttt{reveal\_right}; if taken, send randomization factor and
permutation target index for \texttt{term\_id} row

\item \emph{audit$\rightarrow$halt}: enabled synchronized transition with
Auditor over channel \texttt{audit\_pass}

\item \emph{audit$\rightarrow$caught}: enabled synchronized transition with
Auditor over channel \texttt{audit\_fail}
\end{itemize}

\subsection{Dteller}\label{dteller}

To simulate the theshold decryption, we will use a Shamir's Threshold
scheme. Notice, that here it is possible, that all dtellers refuse to
cooperate, leading to a deadlock. In order to filter this unwanted 
behavior out during property checking we will add a (unconditional) 
fairness assumption, that only 1 out of 3 dtellers can possibly refuse.\medskip

\noindent Private variables:
\begin{itemize}[nosep]
\item \texttt{k\_share} - secret's (private key) share of a
given teller 
\item \texttt{x} - a unique (amongs the tellers) value of first
variable in \texttt{(x,y)} pair (following common practice, for values of 
\texttt{x} we will simply use consecutive numbers from 1)
\end{itemize}\medskip

\noindent States:
\begin{itemize}[nosep]
\item \emph{idle} - waiting for decryption phase
\item \emph{participating} - will cooperate in decryption 
\item \emph{decrypting} - committed state (in-between) for atomic block of statements 
\item \emph{halt} - finished his decryption part 
\item \emph{refused} - refused to cooperate
\end{itemize}\medskip

\noindent Transitions:
\begin{itemize}[nosep] 
\item \emph{idle$\rightarrow$participating}: if number of
cooperating dtellers is low enough, then agree take part in cooperation,
incrementing the number of participants 
\item \emph{participating$\rightarrow$decrypting}: 
if the guard \texttt{dturn} free, change it
to taken and perform decryption procedure.
\item \emph{decrypting$\rightarrow$halt}: another decryption is finished, increment global counter
\texttt{decryption} of decryptions done and free the \texttt{dturn}
guard, permitting next dteller to take his turn
\item \emph{idle$\rightarrow$refused}: refused to cooperate during his turn (while
number of cooperating participants was less than required)
\end{itemize}

\subsection{Sys}\label{sys}

\noindent Private variables:
\begin{itemize}[nosep]  
\item \texttt{vote\_sum} - list of \texttt{|C|} integers, where each \texttt{i}-th
element is a sum of marked votes \texttt{i}-th candidate (tally results)

\item \texttt{ballots\_ready} - as name suggests, a Boolean variable 

\item  \texttt{r\_vec}- (helper variable) integer list of randomization factors, used for
encrypting the seed into onion (ballot generation) 
\item \texttt{r\_ptr }- (helper variable) index of \texttt{r\_vec} element, initially set to 0 
\item \texttt{ballots\_ready }- Boolean value of ``all ballots were generated'' statement
\end{itemize}\medskip

\noindent States:
\begin{itemize}[nosep]
\item  \textit{ballot\_generation} - there are either no ballots or they are
being generating at the moment 
\item \textit{voting }- election phase, when voters
can obtain a ballot form and sumbit their choice 
\item \textit{receipts\_posted }- in-between state, when batch of
receipts is publicly seen, but not processed or decrypted yet
\item \textit{mixing }- wait while mtellers
perform re-encryption mixes 
\item \textit{decryption }- wait while dtellers
perform partial decryption 
\item \textit{results }- receive a batch of onions merged
with indexes, extract original candidate and post results tally
\end{itemize}\medskip

\noindent Transitions:
\begin{itemize}[nosep]

\item \textit{ballot\_generation$\rightarrow$ballot\_generation}
(upper loop): if \texttt{r\_ptr\textgreater{}v\_total} ( \texttt{r\_vec}
is not fully generated ), then enable transition; if it is taken, insert
random factor \texttt{R} into \texttt{r\_vec[r\_ptr]}
and increment \texttt{r\_ptr} by 1.

\item \textit{ballot\_generation$\rightarrow$ballot\_generation} (lower loop): if
\texttt{r\_ptr==v\_total} ( \texttt{r\_vec} is fully generated ) and
ballots are not yet ready (\texttt{!ballots\_ready}), then enable
transition; if it is taken, generate list of ballots using
random values from \texttt{r\_vec} and update \texttt{ballot\_ready}.

\item \textit{ballot\_generation$\rightarrow$voting}: if all ballots were generated
(\texttt{ballot\_ready}), then enable transition; if it is takem, udpate
\texttt{curr\_phase} with relevant phase's code

\item \textit{voting$\rightarrow$voting}: enabled synchronized 
transition with any Voter over channel \texttt{record}; 
if it is taken, read value of shared \texttt{recorded}
receipt, store it in \texttt{initial\_batch} and calculate 
a new onion with absorbed index

\item \textit{voting$\rightarrow$receipts\_posted}: if all voters submitted their
receipts (\texttt{voted==v\_total}), then enable transition; when taken,
update \texttt{curr\_phase} 

\item \textit{receipts\_posted$\rightarrow$mixing}:
allow start of mixing by setting next mix turn to the first mteller
(\texttt{mixes=0})

\item \textit{mixing$\rightarrow$decryption}: if all mixes are
done (\texttt{mixes==mt\_total}) enable transition; if it is  taken, update
\texttt{curr\_phase} and free the guard \texttt{dturn}, allowing
dtellers to perform decryption 

\item \textit{decryption$\rightarrow$results}: if all required decryptions 
are done (\texttt{decryptions==dt\_mit}) enable
transition; if it is taken, update \texttt{curr\_phase}

\item \textit{results$\rightarrow$results}: if results tally have not been posted yet
(\texttt{!results\_ready}), then enable transition; if it is taken, post
results
\end{itemize}
%
%\subsection{Auditor}\label{auditor}
%
%In order not to overflow model with uninteresting subset selection
%procedure (ways of selection k elements of n total) a list of possible
%selection generated in advance (hard-coded in some sense). Thus subset
%selection narrows to selection of element of that list (or it's index).\smallskip
%
%\noindent Private variables:
%\begin{itemize}[nosep]
%\item \emph{comb} - list of possible half of batch
%selections (pre-calculated) 
%\item \emph{curr} - index of currently audited mteller 
%\item \emph{term\_i} - index of batch element that is being checked at the moment 
%\item \emph{pass} - Boolean value, which suggests if the last checked mix-server 
%(instance) passed a correctness check
%\end{itemize}\medskip

%States:
%\begin{itemize}[nosep]
%\item idle 
%\item auditing\_mixes 
%\item auditing\_mix\_i 
%\item choose\_side 
%\item revealed\_left 
%\item revealed\_right 
%\item mix\_fail 
%\item mixes\_pass
%\end{itemize}\medskip

%Transitions:
%\begin{itemize}[nosep] * \emph{-\textgreater{} mix\_fail} - mix-serve
%\texttt{mix\_id} did not pass correctness check and was caught as a
%cheater
%\end{itemize}

\subsection{Optimization}\label{optimization}

To keep model manageable and in attempt to reduce the state space, every
number variable is defined with a possible values bounding.*

One might argue that number of used variables, which also play an
important role in model checking procedure, should be kept strictly
minimal. In our model certain `excess' variables serve a reading
simplicity purpose, despite possible loss of efficiency (which, as we
hope, can be tolerated for the given case-scenario).

*- By default, unbounded integer will use values from -32000 to 32000,
which would carry out a significant impact on the state space

%(?): * format for describing multiple transitions at once and for loops
%     * should naive ballot generation procedure be removed? 
%     * should the audit mix stay? 
%     * italic for states, typewriter for variables, bold for types

%\end{document}

